The Future of Ad Blocking: An Analytical Framework and New Techniques

We present a systematic study of ad blocking - and the associated "arms race" - as a security problem. We model ad blocking as a state space with four states and six state transitions, which correspond to techniques that can be deployed by either publishers or ad blockers. We argue that this is a complete model of the system. We propose several new ad blocking techniques, including ones that borrow ideas from rootkits to prevent detection by anti-ad blocking scripts. Another technique uses the insight that ads must be recognizable by humans to comply with laws and industry self-regulation. We have built prototype implementations of three of these techniques, successfully blocking ads and evading detection. We systematically evaluate our proposed techniques, along with existing ones, in terms of security, practicality, and legality. We characterize the order of growth of the development effort required to create/maintain ad blockers as a function of the growth of the web. Based on our state-space model, our new techniques, and this systematization, we offer insights into the likely "end game" of the arms race. We challenge the widespread assumption that the arms race will escalate indefinitely, and instead identify a combination of evolving technical and legal factors that will determine the outcome.

==> signatureExampleTable.tex <==
\begin{table*}[t]
%\newcommand{\headrow}[1]{\multicolumn{1}{c}{\adjustbox{angle=45,lap=\width-0.5em}{#1}}}
%\newcommand{\full}{$\bullet$}
%\newcommand{\prt}{$\circ$}

% = = = Table bullets: \full and \prt (full and part)
\centering
%\captionsetup{justification=justified}
\begin{tabular}{l  l}
\hline \\[-.7em]
\begin{tabular}{@{}r@{}}Site Match:\\ Expression Match: \\ Expression Replacement: \\ Note:\end{tabular}
&
\begin{tabular}{@{}l@{}}
https?://comunidadiptv.org/ \\ 
\$('\#adsense.an-sponsored .an-advert-banner').outerHeight()===0 \\ 
false \\ 
Example of canceling out the conditional check in an if statement.
\end{tabular}
\\ \hline \\[-.7em]


\begin{tabular}{@{}r@{}}Site Match:\\ Expression Match: \\ Expression Replacement: \\ Note:\end{tabular}
&
\begin{tabular}{@{}l@{}}
(https?://www.elcorreo.com/)$\vert$ (https?://www.lasprovincias.es)$\vert$ (https?://www.larioja.com/) \\ 
typeof Vocento.checkAdBlock=='undefined' \\ 
false \\ 
Example of a replacement on multiple sites.
\end{tabular}
\\ \hline \\[-.7em]

\begin{tabular}{@{}r@{}}Site Match:\\ Expression Match: \\ Expression Replacement: \\ Note:\end{tabular}
&
\begin{tabular}{@{}l@{}}
https?://www.mid-day.com/ \\ 
a.className=``AdSense'' \\ 
a.className=``'' \\ 
Example of replacing a bait string to prevent bait container from being blocked.
\end{tabular}
\\ \hline \\[-.7em]


\begin{tabular}{@{}r@{}}Site Match:\\ Expression Match: \\ Expression Replacement: \\ Note:\end{tabular}
&
\begin{tabular}{@{}l@{}}
https?://www.game-state.com/ \\ 
adblock = true \\ 
adblock = false \\ 
An example of preventing bait variable detection.
\end{tabular}
\\ \hline \\[-.7em]

\end{tabular}

\caption{\label{tab:active_adblocker_rule_examples} Examples of the rules used by the signature-based active ad blocker.}
\end{table*}
